BLADE: ReliaBle Dynamic Hardware-Aware SNN-ANN Boundary SeLection for Event-BAseD Object DEtection

Hybrid Spiking Neural Network (SNN)-Artificial Neural Network (ANN) architectures combine the energy efficiency of SNNs with the superior detection accuracy of ANNs for event-based object detection. Existing hybrid SNN--ANN networks, however, employ static inference and select the SNN-ANN boundary primarily according to accuracy and energy consumption, without considering dynamic inference or reliability. This paper presents BLADE, the first reliability-aware boundary selection methodology for dynamic hybrid SNN-ANN networks with ANN early exit. The proposed framework jointly optimizes the SNN-ANN boundary and ANN early-exit configuration according to reliability, detection accuracy, execution time, and energy consumption, while incorporating reliability through hierarchical statistical fault injection during design-space exploration. Experimental evaluation on an event-based object detector achieves an mAP 0.5 of 0.691 while reducing the inference compute energy to 15.82~mJ when the ANN early exit fires. Reliability analysis identifies the most significant floating-point exponent bit as the dominant source of catastrophic failures, producing significant-or-worse accuracy degradation in 58.8% of its fault injections. Protecting this single bit with approximately 3% storage overhead eliminates catastrophic failures across the evaluated realistic technology fault rates. Furthermore, increasing the proportion of SNN computation improves fault tolerance, with the fully SNN configuration achieving a reliability retention of 0.965 under aggressive fault conditions. The results demonstrate that jointly optimizing reliability, accuracy, execution time, and energy consumption enables more dependable deployment of dynamic hybrid SNN--ANN systems for safety-critical edge AI applications.

==> tables/exit_impact_table.tex <==
%% exit_impact_table.tex -- fault -> exit distribution -> power/latency coupling.
%% Provenance: instance0_results/multibit_ber_dynamic_prot30.exit_impact.json
%% (protect_bits=[30]), region=all. Constants: E_static 16.22 mJ,
%% E_router 1.308 mJ, E_head(skippable) 6.672 mJ, L_full 8.338 ms,
%% L_skippable 0.517 ms. Clean rows = no-fault operating point per arm.
%% dE/dL = fault-induced change vs each arm's own clean point. static and
%% always_exit have dE=dL=0 by construction (no gate to suppress).
%% Delta sub-table columns: the 1.09e-5 anchor (the Riera 16 nm-bulk
%% per-bit rate) is read from the per_bit axis rows of the JSON; the 5e-2
%% saturation column is read from the per_weight axis rows. Verified:
%%   per_bit 1.09e-5 tau_090 -> dE_pct=+0.1620, dL_pct=+0.0248;
%%   per_bit 1.09e-5 tau_092 -> dE_pct=-0.1259 (|0.13|<=0.16), dL_pct=-0.0200 (|0.02|<=0.03);
%%   per_weight 5e-2 tau_090 -> dE_pct=+6.7691, dL_pct=+1.0353;
%%   per_weight 5e-2 tau_092 -> dE_pct=+1.9652, dL_pct=+0.3126.
\begin{table*}[t]
\centering
\caption{Fault coupling to the exit distribution, power, and latency, bit~30 ECC-protected}
\label{tab:exit_impact}
\begin{tabular}{lcccc}
\toprule
\multicolumn{5}{c}{\emph{Clean operating point}} \\
\cmidrule(lr){1-5}
Arm & exit rate & $E$ (mJ) & $L$ (ms) & $P$ (W) \\
\midrule
static       & 0.000 & 16.22 & 8.338 & 1.945 \\
$\tau{=}0.92$ & 0.051 & 17.187 & 8.374 & 2.052 \\
$\tau{=}0.90$ & 0.168 & 16.405 & 8.313 & 1.973 \\
always\_exit & 1.000 & 10.854 & 7.883 & 1.377 \\
\bottomrule
\end{tabular}

\vspace{1.5ex}

\begin{tabular}{lcc}
\toprule
\multicolumn{3}{c}{\emph{Fault-induced} $\Delta E$ / $\Delta L$} \\
\cmidrule(lr){1-3}
Arm & at $1.09{\times}10^{-5}$ (per-bit) & at $5{\times}10^{-2}$ (per-weight) \\
\midrule
static       & $0\%$ / $0\%$ & $0\%$ / $0\%$ \\
$\tau{=}0.92$ & $\le\!0.16\%$ / $\le\!0.03\%$ & $+1.97\%$ / $+0.31\%$ \\
$\tau{=}0.90$ & $+0.162\%$ / $+0.025\%$ & $+6.77\%$ / $+1.04\%$ \\
always\_exit & $0\%$ / $0\%$ & $0\%$ / $0\%$ \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/small_object_table.tex <==
% AUTO-GENERATED by scripts/generate_paper_c1_tables.py from
% size_class_breakdown.json (+ c1_smallobj_ci.py bootstrap block). Do not hand-edit.
\begin{table*}[t]
  \centering
  \caption{Per-size and rare-class recall at the full-model, always-exit, and deployed $\tau{=}0.9$ operating points}
  \label{tab:small_object}
  \begin{tabular}{lccccc}
    \toprule
    Subset & GT boxes & Full & Always-exit & \cellcolor{gray!15}$\tau{=}0.9$ & Drop@$\tau$ \\
    \midrule
    small & $14{,}661$ & 0.669 & 0.601 & \cellcolor{gray!15}0.658 & 0.011 \\
    medium & $23{,}433$ & 0.743 & 0.733 & \cellcolor{gray!15}0.741 & 0.002 \\
    large & $2{,}638$ & 0.680 & 0.644 & \cellcolor{gray!15}0.678 & 0.003 \\
    rare class & $2{,}823$ & 0.582 & 0.362 & \cellcolor{gray!15}0.557 & 0.025 \\
    \bottomrule
  \end{tabular}
\end{table*}

